Using Overlapping Methods to Counter Adversaries in Community Detection

When dealing with large graphs, community detection is a useful data triage tool that can identify subsets of the network that a data analyst should investigate. In an adversarial scenario, the graph may be manipulated to avoid scrutiny of certain nodes by the analyst. Robustness to such behavior is an important consideration for data analysts in high-stakes scenarios such as cyber defense and counterterrorism. In this paper, we evaluate the use of overlapping community detection methods in the presence of adversarial attacks aimed at lowering the priority of a specific vertex. We formulate the data analyst's choice as a Stackelberg game in which the analyst chooses a community detection method and the attacker chooses an attack strategy in response. Applying various attacks from the literature to seven real network datasets, we find that, when the attacker has a sufficient budget, overlapping community detection methods outperform non-overlapping methods, often overwhelmingly so. This is the case when the attacker can only add edges that connect to the target and when the capability is added to add edges between neighbors of the target. We also analyze the tradeoff between robustness in the presence of an attack and performance when there is no attack. Our extensible analytic framework enables network data analysts to take these considerations into account and incorporate new attacks and community detection methods as they are developed.

==> CDMethods.tex <==
\section{Community Detection Methods}
\label{sec:CDmethods}

My approach to this problem will be similar to that for vertex classification in~\cite{Miller2019}: I will consider individual target nodes within datasets where state-of-the-art attack performance has been demonstrated, while also investigating a diverse array of synthetic graphs to learn the context in which these attacks are most and least effective. I will vary the amount of information given about which nodes are of interest, and apply both supervised and unsupervised methods, and attacks against them, to identify where the attacker has the greatest advantage. This will include an investigation into overlapping community detection methods, such as clique percolation~\cite{Palla2005} or edge clustering~\cite{Ahn2010}.

==> simulation.tex <==
\section{Simulation Study}
\label{sec:simulation}
\subsection{Synthetic Dataset Generation}
\subsubsection{Random Graph Models}
We use five random graph models that exhibit different properties in terms of clustering, degree distribution, and dependence on attributes. In each case, we use 4000 nodes and an average degree of approximately 10.
\begin{itemize}
    \item \textbf{Erd\H{o}s--R\'{e}nyi (ER) Graphs}
    \item \textbf{Watts--Strogatz (WS) Graphs}
    \item \textbf{Barab\'{a}si--Albert (BA) Graphs}
    \item \textbf{LFR Graphs}
    \item \textbf{Multiplicative Attribute Graphs (MAGs)}
\end{itemize}
If the generated graph has multiple connected components, we use the largest connected component for the experiment.

\subsubsection{Label Assignment}
We assign labels with varying levels of homophily. For the ``high homophily'' scenario, we partition the nodes based on the normalized graph Laplacian $L=I-D^{-1/2}AD^{-1/2}$, where $A$ and $D$ are the adjacency matrix and diagonal degree matrix as in Section~\ref{sec:model}. We select the eigenvector $u_2$ associated with the second-smallest eigenvalue of $L$. The nodes associated with the $N/2$ entries in $u_2$ with the smallest values (i.e., values closest to $-\infty$) are labeled 0, and the other nodes are labeled 1.\footnote{\todo{I need a good reference for Laplacian-based partitioning.}} Let $V_0$ and $V_1$ be the respective subsets of vertices. 

For lower homophily graphs, we first compute the difference between the number of within-label edges and the number of cross-label edges, i.e., letting $E_{ij}$ be the set of edges between nodes in $V_i$ and nodes in $V_j$,
\begin{equation}
\Delta=|E_{00}|+|E_{11}|-|E_{01}|.
\end{equation}
Depending on how homophilous we want the graph to be, we swap labels on pairs of nodes until $\Delta$ reaches a given value, based on its value from the initial Laplacian-based partition (e.g., half as homophilous as the original). The node swapping mechanism is detailed in Algorithm~\ref{alg:swap}.


\begin{algorithm}
\begin{centering}
\begin{algorithmic}
\STATE \textbf{Input:} Graph $G=(V,E)$, vertex subsets $V_0, V_1$
\STATE \textbf{Output:} Updated vertex subsets $\hat{V}_0, \hat{V}_1$
\STATE $x_i\gets\begin{cases}-1 & \textrm{if }v_i\in V_0\\
1 & \textrm{if }v_i\in V_1\end{cases}$
\STATE $d \gets Ax$
\STATE $p_i\gets d_i\cdot\mathbb{I}[d_i >= 0]\cdot\mathbb{I}[x_i > 0]$
\STATE $u\gets$ node randomly selected with probability $p_i/\sum_{j=1}^N{p_j}$
\STATE $p_i\gets d_i \mathbb{I}[d_i < 0]\mathbb{I}[x_i < 0]$
\STATE $v\gets$ node randomly selected with probability $p_i/\sum_{j=1}^N{p_j}$
\STATE $\hat{V}_0\gets (V_0\cup\{u\})\setminus{v}$
\STATE $\hat{V}_1\gets (V_1\cup\{v\})\setminus{u}$
\RETURN $\hat{V}_0, \hat{V}_1$
\end{algorithmic}
\caption{\textsc{Swap2Reduce}}
\label{alg:swap}
\end{centering}
\end{algorithm}
\subsubsection{Synthetic Attributes}
As with the real graphs, we consider binary attribute vectors on the nodes of the synthetic graphs. In each case, we consider nodes with 100 attributes, and we give each attribute a probability of being true depending on its label. Probabilities are determined by an exponentially decreasing function around We consider three scenarios. In the most difficult case, the probabilities are the same for both classes. As we make the problem easier, we shift the probability function so that attributes with the highest probabilities in one class still have \emph{relatively} high probabilities in the others, but there is not a perfect match. The shift in the probability function is illustrated in Figure~\ref{fig:attributeProb}. The shifts were chosen to create cases where a generalized likelihood ratio test (with each attribute having an independent probability parameter, estimated based on 200 cases for each class) achieves accuracy of approximately $0.5$, $0.7$, and $0.9$. In addition, each node has a one-hot encoded attribute indicating its index in the node set.
\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/attributes.pdf}
    \caption{Caption}
    \label{fig:attributeProb}
\end{figure}

\subsection{Results}
We measure the level of homophily of the resulting labeling by the \emph{heterophilicity} metric
\begin{equation}
H=\frac{\#\{\textrm{edges between $V_0$ and $V_1$}\}}{|V_0||V_1|M/\binom{N}{2}}.\label{eq:heterophilicity}
\end{equation}
The denominator in (\ref{eq:heterophilicity}) is the expected number of edges between $V_0$ and $V_1$ after random rewiring. A high-homophily graph will have relatively low heterophilicity.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/ERBudget.pdf}
    \includegraphics[width=0.45\textwidth]{figures/BABudget.pdf}\\
    \includegraphics[width=0.45\textwidth]{figures/WSBudget.pdf}
    \includegraphics[width=0.45\textwidth]{figures/LFRBudget.pdf}
    \caption{Caption}
    \label{fig:sim_budget}
\end{figure}
